Adaptive Risk Sensitive Model Predictive Control with Stochastic Search

We present a general framework for optimizing the Conditional Value-at-Risk for dynamical systems using stochastic search. The framework is capable of handling the uncertainty from the initial condition, stochastic dynamics, and uncertain parameters in the model. The algorithm is compared against a risk-sensitive distributional reinforcement learning framework and demonstrates outperformance on a pendulum and cartpole with stochastic dynamics. We also showcase the applicability of the framework to robotics as an adaptive risk-sensitive controller by optimizing with respect to the fully nonlinear belief provided by a particle filter on a pendulum, cartpole, and quadcopter in simulation.

==> TODOs.tex <==
1. Replace pdf plots with histograms (Done)
2. Introduce the experiments (discuss the setup)
3. Update the arxiv paper and change the submission to be referring to the arxiv for appendix
4. Move CVaR definition to introduction
5. Add motivation for CVaR in introduction referring to figure 1

==> algorithm_1.tex <==
\begin{algorithm}[H]
\begin{algorithmic}
\State \textbf{Given:} \\
$F$: Transition Model; $K$: Optimization Iterations; $N$: Number of Control Samples; $M$: Number of CVaR Optimization Samples; $T$: Number of timesteps;
$\phi$: System parameters vector; $\alpha_0$: Initial step size; $\alpha_1$: Step size decay rate; $\pi_\eta$: Policy; $\gamma$: Risk level;
\State \textbf{Initialize:}\\ $\theta^0$: natural parameters for policy; $S$: Shape function;

\While{\emph{task not completed}}
    \State $\{x^{ m}_{0}\}_{ m=1,\dots,M} \gets \textit{StateEstimator}()$
    \State $\{\phi^m\}_{m=1,\dots,M}$ $\gets$ $\textit{SampleSystemParameters}()$
    \For{$k$ $\gets$ $1$ to $K$}
        \State $\alpha^k$ $\gets$ $\tfrac{\alpha_{0}}{k^{\alpha_{1}}}$
        \State $\{\eta^{n,k}\}_{n=1,\dots,N}$ $\sim$ $p(\eta ; \theta^k)$
        \For{$n$ $\gets$ $1$ to $N$ \textit{in parallel}}
            \For{$m$ $\gets$ $1$ to $M$ \textit{in parallel}}
                \For{$t$ $\gets$ $0$ to $T-1$}
                    \State $u_{k,t}^{n,m}$ $\sim \pi_{\eta^k}(x^{n,m}_{t})$
                    \State $x_{t+1}^{n,m}\sim p(x_{t+1}^{n,m}|x_t^{n,m}, u_{k,t}^{n,m}; \phi^m)$
                    % \State $\mathcal{J}^{n,m}$ $\mathrel{+}=$ $\textbf{q}(x_{k,t}^{n,m}) + (u_{k,t-1}^{n})^{T}Ru_{k,t-1}^{n}$
                \EndFor
                \State Compute cost: $J^{n,m}(X^{n,m}, U^n_k)$
            \EndFor
            \State $\hat{C}^n \gets \textit{ComputeCVaR}(S(-J^{n,m}), \gamma)$
        \EndFor
        \State $\theta^{k+1}\gets \textit{UpdateParameters}({\hat\{C}^n\}, \alpha^k, \{\eta^{n,k}\})$
    \EndFor
    \State Perform Polyak averaging: $\bar{\theta} \gets \frac{1}{K} \sum_{i=1}^K \theta^i$
    \State Sample policy parameters $\bar{\eta}$ $\sim$ $p(\eta; \bar{\theta})$
    \State Apply policy: $\pi_{\bar{\eta}}$ for $\tau$ timesteps
    \State Recede horizon: $\theta^0 = \omega(\theta^K, \tau)$
    % \For{$t$ $\gets$ $1$ to $T-1$}
    %     \State $\eta^0_{t-1}$ $\gets$ $\eta^K_{t}$ 
    % \EndFor
\EndWhile
\end{algorithmic}
\caption{Stochastic Search for CVaR Optimization}
\label{alg: stochastic_search}
\end{algorithm}

% \begin{algorithm}
% \begin{algorithmic}
% \State \textbf{Given:} \\
% $N$: Number of Control Samples; $M$: Number of CVaR Optimization Samples; $\gamma$: Risk level;
% \For{$n$ $\gets$ $1$ to $N$}
% \State $\mathcal{J}^{n}$ $\gets$ $Sort(\mathcal{J}^{n}, order=descending)$ 
% \State $VaR^{n}$ $\gets$ $\mathcal{J}^{n}[floor(\gamma M)]$
% \State $CVaR^{n}$ $\gets$ $VaR^{n} + \cfrac{1}{M(1 - \gamma)}$ $\sum_{m=1}^{M}$ $\max(0, J^{n,m} - VaR^{n})$
% \EndFor
% \end{algorithmic}
% \caption{Compute CVaR}
% \end{algorithm}


==> algorithm_2.tex <==
\begin{wrapfigure}{R}{0.4\textwidth}
\begin{minipage}{0.4\textwidth}
\vspace{-1 cm}
\begin{algorithm}[H]
\begin{algorithmic}
\State \textbf{Given:} \\
$N$: Number of Control Samples; $\alpha^k$: Stepsize; $\theta^k$: Policy parameters; $\{\eta^k\}$: Policy samples; $\{\hat{C}\}$: CVaR values; $\Pi$: Projection operator for control constraints;
\State $\beta$ $\gets$ $\min(\hat{C})$
\State $\eta$ $\gets$ $\sum_{n=1}^{N}\exp{(-(\hat{C}^{n} - \beta))}$
\For{$n$ $\gets$ $1$ to $N$ \textit{in parallel}}
\State $\omega^{n}$ $\gets$ $\frac{1}{\eta} \exp{(-(\hat{C}^{n} - \beta))}$
% \For{$t$ $\gets$ $0$ to $T-1$}
% \State $u_{t}^{n}$ $\mathrel{+}=$ $u_{t}^{n}w^{n}$
% \EndFor
\State $\nabla_{u}^{n}$ $=$ $\eta^{n} - \frac{1}{N}\sum_{n=1}^N\eta^{n}$
\EndFor
\State $\theta^{k+1}$ $=$ $\Pi\{\theta^{k} + \alpha^k \sum_{n=1}^N \frac{\omega^n\nabla_{u}^{n} }{\eta}\}$
\end{algorithmic}
\caption{Parameter Update}
\label{alg:update_law}
\end{algorithm}
\end{minipage}
\end{wrapfigure}
